Stochastic Deep Networks

Machine learning is increasingly targeting areas where input data cannot be accurately described by a single vector, but can be modeled instead using the more flexible concept of random vectors, namely probability measures or more simply point clouds of varying cardinality. Using deep architectures on measures poses, however, many challenging issues. Indeed, deep architectures are originally designed to handle fixedlength vectors, or, using recursive mechanisms, ordered sequences thereof. In sharp contrast, measures describe a varying number of weighted observations with no particular order. We propose in this work a deep framework designed to handle crucial aspects of measures, namely permutation invariances, variations in weights and cardinality. Architectures derived from this pipeline can (i) map measures to measures - using the concept of push-forward operators; (ii) bridge the gap between measures and Euclidean spaces - through integration steps. This allows to design discriminative networks (to classify or reduce the dimensionality of input measures), generative architectures (to synthesize measures) and recurrent pipelines (to predict measure dynamics). We provide a theoretical analysis of these building blocks, review our architectures' approximation abilities and robustness w.r.t. perturbation, and try them on various discriminative and generative tasks.

==> sections/theory-old.tex <==

%%%
\paragraph{Real-valued map.}
 
% whose proof can be found in Appendix~\ref{sec-proof-approx-thm}, 
The following Theorem shows that any continuous real valued map from random vectors can be approximated to arbitrary precision using two elementary blocks based on fully connected layers. 

\begin{thm}\label{thm-approx}
	Let $\Ff : \Rr(\Omega) \rightarrow \RR$ a continuous map for the convergence in law, where $\Omega \subset \RR^q$ is compact. Then $\forall \epsilon > 0$ there exists two continuous maps $f, g$ such that 
	\eql{\label{eq-approx-thm}
		\forall X \in \Rr(\Omega), \quad \left\lvert \Ff(X) - T_{f} \circ T_{g}(X) \right\rvert \leq \epsilon.
	}
\end{thm}


\begin{proof}
We will prove the theorem for a $T_{g}$ mapping random vectors to deterministic vectors (see Remark~\ref{random-det}) and a $T_f$ mapping this vector to a scalar (see Remark~\ref{rmk-push-fwd}). 
%
We thus aim at proving that 
$\forall \epsilon > 0$, there exist two continuous functions $f,g$ such that 
\eq{
	\forall \al \in \Mm_+^1(\Omega), \quad \left\lvert \Ff(\al) - f \left( \EE_{X \sim \al} \left( g(X) \right) \right) \right\rvert < \epsilon.
}
% Then, functions $h$ and $g$ are approximated by neural networks, and the setting can be rephrased in terms of Elementary Blocks.
% We first approximate any measure $\al \in \Mm_+^1(\Omega)$ by a discretized version on a partition of $\Omega$ using Lemma~\ref{lem-proof-approx-thm} proved below.

Without loss of generality, we assume $\Om \subset [0,1]^d$.
We consider a uniform grid of $N$ points $(x_j)_{j=1}^N$ of $[0,1]^d$, so that the spacing between to consecutive point is $1/N^{1/d}$.
%
We consider the usual piecewise affine P1 finite element basis $(\phi_j)_j$, which are hat functions supported on domains $(S_j)_j$ which are cubes of width $2/N^{1/d}$. 
%
In this setting, $\De_j = \sqrt{d}/N^{1/d}$, so that Lemma~\ref{lem-proof-approx-thm} defines a discrete measure $\hat{\al}_N$ satisfying $\Wass_1( \hat{\al}_N, \al) \leq \sqrt{d}/N^{1/d}$. 


Since $\Om$ is compact, $\Mm_+^1(\Om)$ is compact for the weak$^*$ topology, see~\citep{santambrogio2015optimal}. Since $\Ff$ is weak-$*$ continuous, it is thus uniformly weak$^*$  continuous on $\Mm_+^1(\Om)$. Since  $\hat \al_N \rightharpoonup \al$, $\Ff(\hat{\al}_N) \to \Ff(\al)$ uniformly: there exists $\delta > 0$ s.t. $\forall \al \in \Mm_+^1(\Omega), \Wass_1( \hat{\al}_N, \al) \leq \delta$ implies $\lvert \Ff(\al) - \Ff(\hat{\al}_N) \rvert < \epsilon$. Choosing $N$ large enough such that $\sqrt{d}/N^{1/d} \leq \de$ thus ensures that $\lvert \Ff(\al) - \Ff(\hat{\al}_N) \rvert < \epsilon$.

We now define the following continuous functions
\eq{
	g : 
	x \in \RR^d  \mapsto  \left( \phi_1(x),\hdots,\phi_N(x) \right) \in \RR^N, 
}
\eq{
	\qandq f :  
	(\al_1,..,\al_N) \in \RR^N  \mapsto \Ff ( \sum_{j=1} \al_j \delta_{x_j} ) \in \RR.
}
By construction $\Ff(\hat{\al}_N) = f\left( \EE_{X \sim \al} \left( g(X) \right) \right).$ Hence, \eq{\forall \al \in \Mm_+^1(\Omega), \left\lvert \Ff(\al) - f \left( \EE_{X \sim \al} \left( g(X) \right) \right) \right\rvert < \epsilon.}
\end{proof}



In~\eqref{eq-approx-thm}, $T_{f}$ outputs a constant (deterministic) vector and we abuse notation by assimilating its outputs to its constant value. As explained in Remark~\ref{random-det}, this is achieved by imposing that $f$ only depends on its second argument. 
%
Since $f$ and $g$ are smooth, according to the universality theorem of neural networks~\citep{cybenko1989approximation,leshno1993multilayer} (assuming some restriction on the non-linearity $\la$, namely its being a nonconstant, bounded and continuous function), it is possible to replace each of them (at the expense of increasing $\epsilon$) by a sequence of two fully connected layers (as detailed in Remark~\ref{rem-fully-connected}). This is detailed in Section~\ref{sec-proof-approx-thm} of the appendix. 


%%%
\paragraph{Measure-valued map.}

Similarly, the following Theorem, whose proof can be found in Appendix~\ref{sec-proof-thm-meas-valued} shows that any continuous function mapping random vectors can be approximated to arbitrary precision using three elementary blocks based on fully connected layers, and addition of uniform noise.

\begin{thm}\label{thm-meas-valued}
	Let $\Ff : \Rr(\Xx) \rightarrow \Rr(\Yy)$ a continuous map for the convergence in law, where $\Xx \subset \RR^p$ and $\Yy \subset \RR^q$ are compact. Then $\forall \epsilon > 0$ there exists three continuous maps $f, g, h$ such that 
	\eql{\label{eq-approx-thm}
		\forall X \in \Rr(\Xx), \quad \Wass_1 ( \Ff(X), T_h \circ \Lambda \circ T_{f} \circ T_{g}(X) ) \leq \epsilon.
	}
	where $\Lambda$ is a random noise addition operator.
\end{thm}



    
    \begin{lem}
        $F$ is continuous.
    \end{lem}
    
    \begin{proof}(Lemma)
        Let $\epsilon > 0$ and $a \in \Sigma_{N_\Xx}$. We denote $\hat{a} \eqdef \sum_i a_i \delta_{x_i}$. By continuity of $\Ff$ there exists $\delta > 0$ s.t. $\forall \alpha \in \Mm^1_+(\Xx)$, $\Wass_\Xx(\hat{a}, \alpha) \leq \delta$ implies $\Wass_\Yy(\Ff(\hat{a}),\Ff(\alpha)) \leq \epsilon/\big( \sum_{j=1}^{N_\Yy} \Lip(\phi_j) \big)$. Denoting $d_m = \max_{i=2}^{N_\Xx} \lvert \lvert x_i - x_1 \rvert \rvert_2$, let $\tilde{\delta} = \delta/d_m$. Let $b \in \Sigma_{N_\Xx}$, $\hat{b} \eqdef \sum_i b_i \delta_{x_i}$ s.t. $\lvert \lvert a - b \rvert \rvert_1 < \tilde{\delta}$. Then, 
        \begin{align*}
            \Wass_\Xx(\hat{a},\hat{b}) &= \max_{g \in \Lip(1)} \sum_i (a_i-b_i) g(x_i) \\ &\leq d_m \lvert \lvert a - b \rvert \rvert_1 \leq d_m \tilde{\delta} \leq \delta
        \end{align*}
        since, if $g \in \Lip(1)$, considering without loss of generality that $g(x_1)=0$, then $\forall i, \lvert g(x_i) \rvert \leq d_m$. Hence $\Wass_\Yy(\Ff(\hat{a}),\Ff(\hat{b})) \leq \epsilon/\big( \sum_{j=1}^{N_\Yy} \Lip(\phi_j) \big)$. We end up with:
        \begin{align*}
            \lvert \lvert F(a) - F(b) \rvert \rvert_1 &= \sum_{j=1}^{N_\Yy} \lvert \int_{\Pi_j} \phi_j \mathrm{d}(\Ff(\hat{a})-\Ff(\hat{b})) \rvert \\ &\leq \Wass_\Yy(\Ff(\hat{a}),\Ff(\hat{b})) \sum_{j=1}^{N_\Yy} \Lip(\phi_j) \leq \epsilon
        \end{align*}
        since $\phi_j \geq 0$ and $\phi_j/\Lip(\phi_j) \in \Lip(1)$. Hence the continuity of $F$.
    \end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% OLD %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem~\ref{thm-approx}} \label{sec-proof-approx-thm}

Let us first prove the following:
$\forall \epsilon > 0, \exists$ two continuous functions $h, g$ s.t.
\eq{
\forall \al \in \Mm_+^1(\Omega), \left\lvert \Ff(\al) - g \left( \EE_{X \sim \al} \left( h(X) \right) \right) \right\rvert < \epsilon
}
Then, functions $h$ and $g$ are approximated by neural networks, and the setting can be rephrased in terms of Elementary Blocks.
We first approximate any measure $\al \in \Mm_+^1(\Omega)$ by a discretized version on a partition of $\Omega$ using the following lemma:

\begin{lem}\label{lem-proof-approx-thm}
Let $\left( S_j \right)_{j=1\hdots N}$ be a partition of $\Omega$ ($S_j \subset \RR^d$) and $\left( x_j \right)_{j=1\hdots N}$ representative points in the regions $\left( S_j \right)_{j=1\hdots N}$ respectively.
Let $\left( \phi_j \right)_{j=1..N}$ a set of bounded functions supported respectively on $\left( S_j \right)_{j=1\hdots N}$ such that, $\forall j,$ for any $x \in \mathring{S_j}, \sum_{i=1}^N \phi_i(x) = 1$.
Any measure $\al \in \Mm_+^1(\Omega)$ can be approximated by the weighted sum of atoms $\hat{\al}_N = \sum_{j=1}^N \al_j \delta_{x_j}$ with $\al_j = \int_{S_j} \phi_j(x) \d\al(x)$, and the approximation error is bounded by the largest region diameter (i.e., largest Euclidean distance between two points in the region):
\eq{
\Wass_1 \left( \hat{\al}_N, \al \right) \leq \max_{j=1..N} \text{\upshape diam}(S_j)
}
\end{lem}
%\emph{\color{red}(Since each $\phi_j$ has support $S_j$, on the border of each $S_j$, $\sum_i \phi_i = 0$ so we require $\sum_i \phi_i = 1$ just on the interior of each cell.)}
\begin{proof}
Let $\Pi \in \Mm_+^1(\Omega\times\Omega)$ be a transport plan coupling marginals $\hat{\al}_N$ and $\al$ as follows: $\forall f : \Omega\times\Omega \to \RR,$
\eq{
\int_{\Omega\times\Omega} f \d\Pi = \sum_{j=1}^N \int_{S_j} \phi_j(x) \d\al(x)
}
$\Pi$ indeed is a transport plan: $\forall g : \Omega \to \RR,$
\eq{
\begin{split}
& \int_{\Omega\times\Omega} g(x) \d\Pi(x,y) = \sum_{j=1}^N \int_{S_j} g(x) \phi_j(x) \d\al \\
 &= \sum_{j=1}^N \int_{\Omega} g(x) \phi_j(x) \d\al 
 = \int_{\Omega} g(x) \left( \sum_{j=1}^N \phi_j(x) \right) \d\al \\
 &= \int_{\Omega} g(x) \d\al
\end{split}
}
Also,
\eq{
\begin{split}
&\int_{\Omega\times\Omega} g(y) \d\Pi(x,y) = \sum_{j=1}^N \int_{S_j} g(x_j) \phi_j(x) \d\al \\
 &= \sum_{j=1}^N  g(x_j) \int_{\Omega} \phi_j(x) \d\al 
 = \sum_{j=1}^N  \al_j g(x_j) \\
 &= \int_\Omega g(y) \d\hat{\al}_N
\end{split}
}
By definition of the Wasserstein-1 distance, and using $f(x,y) = \norm{x-y}_1$,
\eq{
\begin{split}
\Wass(\hat{\al}_N,\al) & \leq \int_{\Omega\times\Omega} \norm{x-y}_1 \d\Pi(x,y) \\
& = \sum_{j=1}^N \int_{S_j} \phi_j(x) \norm{x-x_j}_1 \d\al(x) \\
& \leq \sum_{j=1}^N \int_{S_j} \phi_j(x) \text{diam}(S_j) \d\al(x) \\
& \leq \left( \sum_{i=1}^N \int_{\Omega} \phi_i(x) \d\al(x) \right) \max_{j=1}^N \text{diam}(S_j) \\
& = \max_{j=1}^N \text{diam}(S_j)
\end{split}
}
\end{proof}

We consider as regions $(S_j)_{j=1\hdots N}$ a regular grid, and take as $(\phi_j)_{j=1\hdots N}$ a collection of (continuous) separable triangle functions in these regions respectively (triangle functions in 1D, product of triangle functions along each dimension otherwise). In this setting, $\text{diam}(S_j) \leq \frac{2}{N^{\frac{1}{d}}}$. Hence, as $N \to +\infty$, $\Wass_1 \left( \hat{\al}_N, \al \right) \to 0$. Moreover, $f$ is weak-$*$ continuous on a compact set, therefore Heine theorem yields $f(\hat{\al}_N) \to_{N\to\infty} \Ff(\al)$ uniformly: let $\epsilon > 0$, there exists $\delta > 0$ s.t. $\forall \al \in \Mm_+^1(\Omega), \Wass_1 \left( \hat{\al}_N, \al \right) \leq \delta$ implies $\left\lvert \Ff(\al) - f(\hat{\al}_N) \right\rvert < \epsilon$ (with $N = \floor{\left( \frac{2}{\delta} \right)^d}+1$ for instance).
Let the continuous functions
\eq{
	h : 
	x \in \RR^d  \mapsto  \left( \la(x),\hdots,\phi_N(x) \right) \in \RR^N
}
and
\eq{
	g :  
	(\al_1,..,\al_N) \in \RR^N  \mapsto f \Big( \sum_{j=1}^N \al_j \delta_{x_j} \Big) \in \RR 
}
It is straightforward that $f(\hat{\al}_N) = g \left( \EE_{X \sim \al} \left( h(X) \right) \right).$ Hence, \eq{\forall \al \in \Mm_+^1(\Omega), \left\lvert \Ff(\al) - g \left( \EE_{X \sim \al} \left( h(X) \right) \right) \right\rvert < \epsilon.}

We now approximate continuous functions $g$ and $h$ by neural networks. Namely, let us prove that: $\forall \epsilon > 0$, there exists whole numbers $N, p_1, p_2$; pointwise nonlinearities $\la, \la$; weight matrices matrices $A_1 \in \RR^{d \times p_1}$, $A_2 \in \RR^{N \times p_2}$, $C_1 \in \RR^{p_1 \times N}$, $C_2 \in \RR^{p_2 \times 1}$; biases $b_1 \in \RR^{p_1}$, $b_2 \in \RR^{p_2}$: i.e., there exists two neural networks:
\begin{itemize}
	\item $h_\theta(x) = C_1^\intercal \la (A_1^\intercal x + b_1) : \RR^d \to \RR^N$
	\item $g_\xi(x) = C_2^\intercal \la (A_2^\intercal x + b_2) : \RR^N \to \RR$
\end{itemize}
s.t.
\eq{
\forall \al \in \Mm_+^1(\Omega), \left\lvert \Ff(\al) - g_\xi \left( \EE_{X \sim \al} \left( h_\theta(X) \right) \right) \right\rvert < \epsilon
}

Let $\epsilon > 0$. By theorem 1, $f$ can be approximated arbitrarily close (up to $\frac{\epsilon}{3}$) by a composition of functions of the form $g \left( \EE_{X \sim \al} \left( h(X) \right) \right)$. By triangular inequality, we upper-bound the difference of interest $\left\lvert \Ff(\al) - g_\xi \left( \EE_{X \sim \al} \left( h_\theta(X) \right) \right) \right\rvert$ by a sum of three terms:
\begin{itemize}
	\item $\left\lvert \Ff(\al) - g \left( \EE_{X \sim \al} \left( h(X) \right) \right) \right\rvert$
	\item $\left\lvert g \left( \EE_{X \sim \al} \left( h(X) \right) \right) - g_\xi \left( \EE_{X \sim \al} \left( h(X) \right) \right) \right\rvert$
	\item $\left\lvert g_\xi \left( \EE_{X \sim \al} \left( h(X) \right) \right) - g_\xi \left( \EE_{X \sim \al} \left( h_\theta(X) \right) \right) \right\rvert$
\end{itemize}
and bound each term by $\frac{\epsilon}{3}$, which yields the result.
The bound on the first term directly comes from theorem 1 and yields constant $N$ which depends on $\epsilon$. The bound on the second term is a direct application of the universal approximation theorem (since $\al$ is a probability measure, input values of $g$ lie in a compact subset of $\RR^N$: indeed, $\left\left \int_\Omega h(x) \mathrm{d}\alpha \right\right_\infty \leq \max_{x\in\Omega} \max_i \left h_i(x) \right$ --- hence the theorem is applicable). Let us focus on the third term.
Continuity of $g_\xi$ yields the existence of $\delta > 0$ s.t. $\left\lvert \left\lvert x-y \right\rvert \right\rvert_1 < \delta$ implies $\left\lvert g_\xi(x)-g_\xi(y) \right\rvert < \frac{\epsilon}{3}$. Let us apply the universal approximation theorem: each component $h_i$ of $h$ can be approximated by a neural network $h_{\theta,i}$ up to $\frac{\delta}{N}$. Therefore:
\eq{
\begin{split}
\lvert \lvert \EE_{X \sim \al} & \left( h(X) - h_\theta(X) \right) \rvert \rvert_1 \\
& \leq \EE_{X \sim \al} \lvert \lvert h(X) - h_\theta(X) \rvert \rvert_1 \\
& \leq \sum_{i=1}^N \int_\Omega \lvert h_i(x) - h_{\theta,i}(x) \rvert \d\al(x) \\
& \leq N \times \frac{\delta}{N} = \delta
\end{split}
}
since $\al$ is a probability measure. Hence the bound on the third term.



\fi %%% REMOVED %%%%

% \newpage




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem~\ref{thm-meas-valued}}
\label{sec-proof-thm-meas-valued}

Without loss of generality, we assume $\Xx \subset [0;1]^p$ and $\Yy \subset [0;1]^q$. We consider a uniform grid of $N_\Xx$ points $(x_i)_{i=1}^{N_\Xx}$ of $[0,1]^p$ and $N_\Yy$ points $(y_j)_{j=1}^{N_\Yy}$ of $[0,1]^q$. We consider a partition $\left( S_i \right)_{i=1}^{N_\Xx}$ of $[0,1]^p$, with $x_i \in S_i$ (resp, a partition $\left( \Pi_j \right)_{j=1}^{N_\Yy}$ of $[0,1]^q$, with $y_j \in \Pi_j$). Let $\Sigma_n = \{ (a_i)_{i=1..n} \in \RR^n : \sum_{i=1}^n a_i=1, a_i \geq 0 \}$.
    
    \noindent Let $F: a \in \Sigma_{N_\Xx} \mapsto D_\Yy \big( \Ff(\sum_{j=1}^{N_\Yy} a_i \delta_{x_i} ) \big) \in \Sigma_{N_\Yy}$, where $D_\Yy : \alpha \in \Mm^1_+(\Yy) \mapsto \big( \int_{\Sigma_j} \phi_j \mathrm{d}\alpha \big)_{j=1..N_\Yy} \in \RR^{N_\Yy}$ is the discretization operator according to partition $\left( \Pi_j \right)_{j=1}^{N_\Yy}$, with $(\phi_j)_j$ the piecewise affine P1 finite element basis. Similarly, we denote $D_\Xx$ the discretization operator of measures on $[0;1]^p$ according to partition $(S_i)_{i=1}^{N_\Xx}$.
    
    \begin{lem}
        $F$ is continuous.
    \end{lem}
    
    \begin{proof}(Lemma)
        Let $\epsilon > 0$ and $a \in \Sigma_{N_\Xx}$. We denote $\hat{a} \eqdef \sum_i a_i \delta_{x_i}$. By continuity of $\Ff$ there exists $\delta > 0$ s.t. $\forall \alpha \in \Mm^1_+(\Xx)$, $\Wass_\Xx(\hat{a}, \alpha) \leq \delta$ implies $\Wass_\Yy(\Ff(\hat{a}),\Ff(\alpha)) \leq \epsilon/\big( \sum_{j=1}^{N_\Yy} \Lip(\phi_j) \big)$. Denoting $d_m = \max_{i=2}^{N_\Xx} \lvert \lvert x_i - x_1 \rvert \rvert_2$, let $\tilde{\delta} = \delta/d_m$. Let $b \in \Sigma_{N_\Xx}$, $\hat{b} \eqdef \sum_i b_i \delta_{x_i}$ s.t. $\lvert \lvert a - b \rvert \rvert_1 < \tilde{\delta}$. Then, 
        \begin{align*}
            \Wass_\Xx(\hat{a},\hat{b}) &= \max_{g \in \Lip(1)} \sum_i (a_i-b_i) g(x_i) \\ &\leq d_m \lvert \lvert a - b \rvert \rvert_1 \leq d_m \tilde{\delta} \leq \delta
        \end{align*}
        since, if $g \in \Lip(1)$, considering without loss of generality that $g(x_1)=0$, then $\forall i, \lvert g(x_i) \rvert \leq d_m$. Hence $\Wass_\Yy(\Ff(\hat{a}),\Ff(\hat{b})) \leq \epsilon/\big( \sum_{j=1}^{N_\Yy} \Lip(\phi_j) \big)$. We end up with:
        \begin{align*}
            \lvert \lvert F(a) - F(b) \rvert \rvert_1 &= \sum_{j=1}^{N_\Yy} \lvert \int_{\Pi_j} \phi_j \mathrm{d}(\Ff(\hat{a})-\Ff(\hat{b})) \rvert \\ &\leq \Wass_\Yy(\Ff(\hat{a}),\Ff(\hat{b})) \sum_{j=1}^{N_\Yy} \Lip(\phi_j) \leq \epsilon
        \end{align*}
        since $\phi_j \geq 0$ and $\phi_j/\Lip(\phi_j) \in \Lip(1)$. Hence the continuity of $F$.
    \end{proof}
    
    For any $b \in \Sigma_{N_\Yy}$, we consider the optimal transport map $\theta_b$ from the uniform probability measure on $\Yy$ to $(1-\epsilon) \sum_{i=1..N_\Yy} b_i \delta_{z_i} + \epsilon$ where $(z_i)_{i=1\cdots N_\Yy}$ is a uniform $q$-dimensional sample according to grid $(\Pi_j)_{j=1\cdots N_\Yy}$ ($\forall i, z_i$ is sampled uniformly on $\Pi_i$, which operation we denote $\Lambda$). We define $f:[0;1]^p\times [0;1]^p \to \RR^{N_\Xx}, (x,y) \mapsto (\phi_i(y))_{i=1\cdots N_\Xx}$, $g: \Sigma_{N_\Xx} \times \Sigma_{N_\Xx} \to \Sigma_{N_\Yy}, (x,y) \mapsto F(y)$ and $h: \RR^{N_\Yy+q} \times \RR^{N_\Yy+q} \to \RR^q, ([z;b],[w;c]) \mapsto \theta_b(z)$. By continuity of $\phi_i$ and $F$, $f$ and $g$ are continuous.

    \begin{lem}
    $h$ is continuous in both variables.
    \end{lem}
    
    \begin{proof}
        TO DO
    \end{proof}
    
    We end up with $\Wass_\Yy(\Ff(\alpha), T_h \circ \Lambda \circ T_{f} \circ T_{g}(\alpha)) \leq \Wass_\Yy(\Ff(\alpha), \Ff(D_\Xx(\alpha))) + \Wass_\Yy(\Ff(D_\Xx(\alpha)), T_h \circ \Lambda \circ T_{f} \circ T_{g}(\alpha))$. Similarly as in Theorem~\ref{thm-approx}, choosing $N_\Xx$ large enough ($\frac{1}{N_\Xx^{1/p}} < \delta$ wtih same notations) ensures that $\Wass_\Yy(\Ff(\alpha), \Ff(D_\Xx(\alpha)))$ is small enough ($< \epsilon$) by Lemma~\ref{lem-proof-approx-thm} and uniform continuity of $\Ff$. Using again Lemma~\ref{lem-proof-approx-thm}, as long as $\frac{1}{N_\Yy^{1/q}} < \epsilon$, $\Wass_\Yy(\Ff(D_\Xx(\alpha)), T_h \circ \Lambda \circ T_{f} \circ T_{g}(\alpha)) < \epsilon$.
    
    
    
  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Proof of Proposition~\ref{prop-tensorization}}\label{sec-proof-prop-tensorization}
%
%
%	One has
%	\eq{
%	\begin{split}
%		 &\Wass_{\Xx \times \Yy}( \al \otimes \be,  \al' \otimes \be' )  \\
%		&= \umax{\Lip(g)\leq 1}
%			\int_{\Xx \times \Yy} g(x,y) [ \d\al(x)\d\be(y)-\d\al'(x)\d\be'(y) ] \\
%		& = 
%		\umax{\Lip(g)\leq 1}
%		\int_\Xx \int_\Yy g(x,y)[\d\be(y)-\d\be'(y)]\d\al(x) \\
%		& +   
%		\int_\Yy \int_\Xx g(x,y)[\d\al(x)-\d\al'(x)]\d\be(y),
%	\end{split}
%	}
%	hence the result.

